Large-angle production of charged pions by 3 GeV/c - 12 GeV/c protons on carbon, copper and tin targets

A measurement of the double-differential $\pi^{\pm}$ production cross-section in proton--carbon, proton--copper and proton--tin collisions in the range of pion momentum $100 \MeVc \leq p < 800 \MeVc$ and angle $0.35 \rad \le \theta <2.15 \rad$ is presented. The data were taken with the HARP detector in the T9 beam line of the CERN PS. The pions were produced by proton beams in a momentum range from 3 \GeVc to 12 \GeVc hitting a target with a thickness of 5% of a nuclear interaction length. The tracking and identification of the produced particles was done using a small-radius cylindrical time projection chamber (TPC) placed in a solenoidal magnet. An elaborate system of detectors in the beam line ensured the identification of the incident particles. Results are shown for the double-differential cross-sections at four incident proton beam momenta (3 \GeVc, 5 \GeVc, 8 \GeVc and 12 \GeVc).

==> Cu5-Sn5_table1.tex <==
% copper (tin) 
\begin{table}[tbp!] 
\caption{Total number of events and tracks used in the copper (tin) 
  5\%~$\lambda_{\mathrm{I}}$ target data set, and the number of
  protons on target as calculated from the pre-scaled trigger count.} 
\label{tab:events}
{\small
\begin{center}
\begin{tabular}{ l  r  r r r} \hline
\bf{Data set}&\bf{3 \bfGeVc}&\bf{5 \bfGeVc}&\bf{8 \bfGeVc}&\bf{12 \bfGeVc}\\ \hline
    Total DAQ events                        & 992549 (1636933)   & 2166883 (2827930) & 2599056 (2780036) &  748123 (950582) \\
    Protons on target                               & 971840 (1379008)   & 3626048 (4598848) & 7606272 (8260544) & 2990656 (3842112) \\
     (selected min. bias$\times$64)              &                    &                   &                   &                 \\ 
    Acc. protons with LAI        &  59873 (83549) &  237894 (304949) &  541852 (600581) &  226250 (295053)  \\
    Maximum \evtspill                                   &    130 (110)  &     120 (110)  &     120 (120)  &     130 (110) \\
    LAI in accepted spill part                    &  27287 (30029) &   87974 (98078) &  175770 (199209) &   90752 (100872) \\
    Fraction of triggers used                           &   46\% (36 \%)  &    37\% (32 \%)  &    32\% (33\%)  &    40\% (34\%) \\
    Acc. mom. (vtx constr.)               &  37681 (42949)  &  156847 (188994)   &  374701 (481436) &  209043 (274700) \\
    In kin. region, from target                 &  23896 (29090) &   99652  (125864) &  229002 (305214) &  122273 (167137) \\
    Negative particles                                  &   3016 (3352)  &   18242 (20721) &   52447 (63846) &   31239 (39395) \\
    Positive particles                                  &  20880 (25738) &   81410 (105143) &  176555 (241368) &   91034 (127742) \\
    \bf{$\bfpim$ selected with PID}                     &   2728 (3100)  &   16451 (18762) &   46820 (56697) &   27636 (34595) \\
    \bf{$\bfpip$ selected with PID}                     &   4403 (4439) &   22087 (23402) &   57218 (64410) &   32234 (38009) \\
\end{tabular}
\end{center}
}
\end{table}
% counters of target.py used:
% #11
% #41 x64
% #21
% #22
% nevt
% #23
% #23/#22
% #72
% mult (mean of trk_mult1 in ..target.aida)
% #84
% #87
% #91
% #92
% #88
% #89




==> Cu5_syst-table.tex <==
% copper 
\begin{table}[tbp!] 
\small{
\begin{center}
\caption{Contributions to the experimental uncertainties for the copper analysis. The numbers
  represent the uncertainty in percent of 
  the cross-section integrated over the angle and momentum region indicated.} 
\label{tab:errors-3}
\vspace{2mm}
\begin{tabular}{ l rrr | rrr | rr} \hline
\bf{Momentum range  (\MeVc)}&\multicolumn{3}{c|}{100 -- 300}
                            &\multicolumn{3}{c|}{300 -- 500}
                            &\multicolumn{2}{c}{500 -- 700} \\
\hline
\bf{Angle range (\rad)}&0.35--&0.95--&1.55--
                       &0.35--&0.95--&1.55--
                       &0.35--&0.95-- \\
\bf{Error source}      &0.95&1.55&2.15
                       &0.95&1.55&2.15
                       &0.95&1.55 \\
%3
\hline
\bf{3 \GeVc beam}&&&&&&&&\\
\hline
Absorption                & 1.3 & 1.6 & 1.9 & 0.6 & 0.4 & 0.1 & 0.3 & 0.4 \\
Tertiaries                & 3.3 & 4.4 & 4.8 & 2.6 & 2.4 & 0.9 & 0.3 & 0.5 \\
Target region cut         & 2.3 & 0.8 & 0.7 & 0.8 & 0.5 & 1.2 & 2.7 & 0.9 \\
Efficiency                & 1.5 & 2.2 & 1.0 & 1.5 & 2.8 & 2.8 & 1.9 & 3.3 \\
Shape of $\pi^0$          & 5.0 & 2.1 & 0.3 & 0.2 & 0.1 & 0.2 & 0.0 & 0.0 \\
Normalization of $\pi^0$  & 3.1 & 1.9 & 1.1 & 0.1 & 0.1 & 0.1 & 0.0 & 0.0 \\
Particle ID               & 0.1 & 0.0 & 0.0 & 1.1 & 0.7 & 0.1 & 5.4 & 4.8 \\
Momentum resolution       & 2.6 & 1.8 & 1.1 & 0.2 & 0.0 & 0.4 & 0.3 & 0.4 \\
Momentum scale            & 7.1 & 4.7 & 2.7 & 0.9 & 6.2 & 8.6 & 7.6 &11.2 \\
Angle bias                & 1.1 & 0.4 & 0.1 & 0.2 & 1.1 & 1.5 & 1.0 & 1.9 \\
\bf{Total systematics}    &10.7 & 7.8 & 6.2 & 3.5 & 7.3 & 9.3 &10.0 &12.8 \\
\bf{Statistics}           & 5.1 & 4.4 & 5.2 & 4.0 & 6.1 &15.1 & 5.3 &12.4 \\
%5
\hline
\bf{5 \GeVc beam}&&&&&&&&\\
\hline
Absorption                & 1.3 & 1.6 & 1.8 & 0.5 & 0.4 & 0.1 & 0.3 & 0.5 \\
Tertiaries                & 3.2 & 4.4 & 4.5 & 2.6 & 2.5 & 1.4 & 0.3 & 0.5 \\
Target region cut         & 2.7 & 1.5 & 1.4 & 1.6 & 0.6 & 1.4 & 1.2 & 0.7 \\
Efficiency                & 1.9 & 2.5 & 1.9 & 1.4 & 2.5 & 2.7 & 1.6 & 3.1 \\
Shape of $\pi^0$          & 4.2 & 1.0 & 0.5 & 0.1 & 0.1 & 0.2 & 0.0 & 0.0 \\
Normalization of $\pi^0$  & 3.4 & 2.2 & 1.4 & 0.2 & 0.1 & 0.1 & 0.0 & 0.0 \\
Particle ID               & 0.1 & 0.0 & 0.0 & 1.0 & 0.6 & 0.3 & 5.1 & 4.4 \\
Momentum resolution       & 2.6 & 1.6 & 1.5 & 0.1 & 0.1 & 0.9 & 0.1 & 0.6 \\
Momentum scale            & 7.1 & 4.8 & 3.4 & 0.9 & 3.7 & 5.4 & 4.2 &11.1 \\
Angle bias                & 0.9 & 0.5 & 0.1 & 0.2 & 1.2 & 0.7 & 1.0 & 1.9 \\
\bf{Total systematics}    &10.5 & 7.9 & 6.8 & 3.6 & 5.3 & 6.5 & 7.0 &12.6 \\
\bf{Statistics        }   & 2.2 & 2.0 & 2.5 & 1.7 & 2.4 & 4.4 & 2.0 & 3.7 \\
%8
\hline
\bf{8 \GeVc beam}&&&&&&&&\\
\hline
Absorption                & 1.3 & 1.5 & 1.7 & 0.6 & 0.4 & 0.1 & 0.3 & 0.6 \\
Tertiaries                & 3.0 & 4.2 & 4.0 & 2.6 & 2.7 & 1.5 & 0.4 & 0.3 \\
Target region cut         & 3.0 & 1.9 & 1.4 & 2.1 & 0.4 & 0.2 & 1.2 & 0.3 \\
Efficiency                & 1.6 & 2.1 & 1.6 & 1.1 & 2.0 & 2.3 & 1.2 & 2.2 \\
Shape of $\pi^0$          & 3.0 & 0.7 & 0.3 & 0.1 & 0.1 & 0.1 & 0.0 & 0.0 \\
Normalization of $\pi^0$  & 4.4 & 2.5 & 1.6 & 0.2 & 0.1 & 0.1 & 0.0 & 0.0 \\
Particle ID               & 0.0 & 0.0 & 0.0 & 1.1 & 0.5 & 0.2 & 5.1 & 4.1 \\
Momentum resolution       & 2.6 & 1.7 & 2.1 & 0.0 & 0.4 & 0.2 & 0.1 & 0.6 \\
Momentum scale            & 7.0 & 4.5 & 4.0 & 1.7 & 2.2 & 5.0 & 3.5 & 8.8 \\
Angle bias                & 0.7 & 0.5 & 0.0 & 0.4 & 1.2 & 1.0 & 0.9 & 1.7 \\
\bf{Total systematics}    &10.4 & 7.6 & 6.8 & 4.1 & 4.3 & 5.8 & 6.5 &10.2 \\
\bf{Statistics}           & 1.4 & 1.3 & 1.6 & 1.0 & 1.4 & 2.6 & 1.2 & 2.1 \\
%12
\hline
\bf{12 \GeVc beam}&&&&&&&&\\
\hline
Absorption                & 1.2 & 1.3 & 1.6 & 0.5 & 0.4 & 0.1 & 0.3 & 0.5 \\
Tertiaries                & 0.6 & 3.2 & 3.5 & 1.1 & 1.9 & 0.5 & 1.0 & 0.2 \\
Target region cut         & 4.2 & 2.9 & 1.6 & 2.5 & 1.0 & 0.4 & 2.2 & 0.2 \\
Efficiency                & 1.7 & 2.4 & 2.1 & 1.2 & 2.2 & 2.4 & 1.1 & 2.5 \\
Shape of $\pi^0$          & 3.0 & 0.2 & 1.3 & 0.1 & 0.1 & 0.2 & 0.0 & 0.0 \\
Normalization of $\pi^0$  & 4.0 & 2.5 & 1.6 & 0.2 & 0.1 & 0.1 & 0.1 & 0.0 \\
Particle ID               & 0.1 & 0.2 & 0.2 & 1.0 & 0.5 & 0.1 & 5.1 & 4.0 \\
Momentum resolution       & 2.6 & 2.1 & 2.2 & 0.2 & 0.5 & 0.6 & 0.3 & 0.7 \\
Momentum scale            & 7.6 & 5.0 & 4.2 & 1.7 & 2.1 & 5.5 & 3.2 &10.0 \\
Angle bias                & 0.6 & 0.5 & 0.1 & 0.4 & 1.4 & 0.7 & 0.9 & 1.9 \\
\bf{Total systematics}    &10.6 & 7.9 & 7.0 & 3.6 & 4.1 & 6.1 & 6.6 &11.3 \\
\bf{Statistics}           & 1.7 & 1.7 & 2.1 & 1.3 & 1.9 & 3.5 & 1.4 & 2.7 \\
\end{tabular}
\end{center}
}
\end{table}






















































==> Cu5_table1.tex <==
% copper 
\begin{table}[tbp!] 
\caption{Total number of events and tracks used in the copper 
  5\%~$\lambda_{\mathrm{I}}$ target data sets, and the number of
  protons on target as calculated from the pre-scaled trigger count.} 
\label{tab:events}
\begin{center}
\begin{tabular}{ l  r  r r r} \hline
\bf{Data set}&\bf{3 \bfGeVc}&\bf{5 \bfGeVc}&\bf{8 \bfGeVc}&\bf{12 \bfGeVc}\\ \hline
    Total events taken by the DAQ                       & 992549  & 2166883  & 2599056  &  748123  \\
    Protons on target (selected minimum bias$\times$64) & 971840  & 3626048  & 7606272  & 2990656  \\
    Accepted protons with interaction triggers          & 145915  &  467809  &  969364  &  385923  \\
    Accepted protons with Large Angle Int. (LAI)        &  59873  &  237894  &  541852  &  226250  \\
    Maximum \evtspill                                   &    130  &     120  &     120  &     130  \\
    LAI in accepted part of the spill                   &  27287  &   87974  &  175770  &   90752  \\
    Fraction of triggers used                           &   46\%  &    37\%  &    32\%  &    40\%  \\
    LA tracks with $\ge 12$ hits                        &  50401  &  215905  &  521599  &  300643  \\
    Average multiplicity                                &    2.4  &     3.2  &     4.2  &     4.9  \\
    Accepted momentum (vertex constraint)               &  37681  &  156847  &  374701  &  209043  \\
    From target and in kinematic region                 &  23896  &   99652  &  229002  &  122273  \\
    Negative particles                                  &   3016  &   18242  &   52447  &   31239  \\
    Positive particles                                  &  20880  &   81410  &  176555  &   91034  \\
    \bf{$\bfpim$ selected with PID}                     &   2728  &   16451  &   46820  &   27636  \\
    \bf{$\bfpip$ selected with PID}                     &   4403  &   22087  &   57218  &   32234  \\
\end{tabular}
\end{center}
\end{table}
% counters of target.py used:
% #11
% #41 x64
% #21
% #22
% nevt
% #23
% #23/#22
% #72
% mult (mean of trk_mult1 in ..target.aida)
% #84
% #87
% #91
% #92
% #88
% #89




==> Sn5_syst-table.tex <==
% tin 
\begin{table}[tbp!] 
\small{
\begin{center}
\caption{Contributions to the experimental uncertainties for the tin analysis. The numbers
  represent the uncertainty in percent of 
  the cross-section integrated over the angle and momentum region indicated.} 
\label{tab:errors-3}
\vspace{2mm}
\begin{tabular}{ l rrr | rrr | rr} \hline
\bf{Momentum range  (\MeVc)}&\multicolumn{3}{c|}{100 -- 300}
                            &\multicolumn{3}{c|}{300 -- 500}
                            &\multicolumn{2}{c}{500 -- 700} \\
\hline
\bf{Angle range (\rad)}&0.35--&0.95--&1.55--
                       &0.35--&0.95--&1.55--
                       &0.35--&0.95-- \\
\bf{Error source}      &0.95&1.55&2.15
                       &0.95&1.55&2.15
                       &0.95&1.55 \\
%3
\hline
\bf{3 \GeVc beam}&&&&&&&&\\
\hline
Absorption                & 1.0 & 1.2 & 1.6 & 0.5 & 0.3 & 0.1 & 0.4 & 0.4  \\
Tertiaries                & 2.4 & 3.5 & 3.6 & 2.3 & 2.1 & 0.9 & 0.1 & 0.4  \\
Target region cut         & 0.9 & 1.3 & 0.1 & 0.7 & 0.7 & 0.8 & 1.4 & 0.8  \\
Efficiency                & 1.5 & 1.9 & 1.5 & 1.7 & 3.2 & 2.5 & 2.1 & 3.2  \\
Shape of $\pi^0$          &10.5 & 3.1 & 0.1 & 0.4 & 0.1 & 0.3 & 0.0 & 0.0  \\
Normalization of $\pi^0$  & 3.4 & 1.9 & 1.2 & 0.2 & 0.1 & 0.1 & 0.0 & 0.0  \\
Particle ID               & 0.2 & 0.1 & 0.0 & 1.2 & 0.7 & 0.1 & 5.5 & 4.1  \\
Momentum resolution       & 1.8 & 0.1 & 0.8 & 0.3 & 0.7 & 1.5 & 0.1 & 0.3  \\
Momentum scale            & 7.3 & 2.5 & 1.3 & 1.1 & 4.7 &11.2 & 4.7 &11.2  \\
Angle bias                & 0.8 & 0.3 & 0.3 & 0.2 & 1.2 & 0.9 & 0.8 & 1.4  \\
\bf{Total systematics}    &13.7 & 6.2 & 4.6 & 3.4 & 6.3 &11.7 & 7.7 &12.4  \\
\bf{Statistics}           & 4.9 & 4.1 & 5.0 & 4.3 & 6.5 &14.1 & 5.6 &12.0  \\
%5
\hline
\bf{5 \GeVc beam}&&&&&&&&\\
\hline
Absorption               & 1.1 & 1.2 & 1.5 & 0.5 & 0.3 & 0.2 & 0.3 & 0.4  \\
Tertiaries               & 2.7 & 3.5 & 3.6 & 2.2 & 2.6 & 1.8 & 0.3 & 0.2  \\
Target region cut        & 2.4 & 1.5 & 1.7 & 1.7 & 0.4 & 0.2 & 1.0 & 0.5  \\
Efficiency               & 1.7 & 2.0 & 1.4 & 1.6 & 2.3 & 3.0 & 1.6 & 2.5  \\
Shape of $\pi^0$         & 5.3 & 1.3 & 0.1 & 0.2 & 0.1 & 0.2 & 0.0 & 0.0  \\
Normalization of $\pi^0$ & 3.7 & 2.3 & 1.5 & 0.2 & 0.1 & 0.1 & 0.0 & 0.0  \\
Particle ID              & 0.1 & 0.1 & 0.1 & 1.0 & 0.7 & 0.3 & 5.2 & 4.3  \\
Momentum resolution      & 1.4 & 0.1 & 0.4 & 0.1 & 0.9 & 1.2 & 0.2 & 1.4  \\
Momentum scale           & 5.6 & 2.9 & 1.6 & 0.7 & 2.9 & 5.8 & 4.5 &11.9  \\
Angle bias               & 0.9 & 0.5 & 0.1 & 0.1 & 1.2 & 1.2 & 0.8 & 1.5  \\
\bf{Total systematics}   & 9.7 & 6.0 & 5.0 & 3.5 & 4.8 & 7.0 & 7.2 &13.1  \\
\bf{Statistics        }  & 2.1 & 1.8 & 2.2 & 1.7 & 2.4 & 4.3 & 2.1 & 3.6  \\
%8
\hline
\bf{8 \GeVc beam}&&&&&&&&\\
\hline
Absorption                & 1.1 & 1.2 & 1.5 & 0.5 & 0.4 & 0.3 & 0.4 & 0.4  \\
Tertiaries                & 2.5 & 3.4 & 3.6 & 2.3 & 2.7 & 2.5 & 0.1 & 0.2  \\
Target region cut         & 2.7 & 1.9 & 0.4 & 1.9 & 0.3 & 0.4 & 1.2 & 0.2  \\
Efficiency                & 1.5 & 2.2 & 1.1 & 1.3 & 2.1 & 1.9 & 1.5 & 2.2  \\
Shape of $\pi^0$          & 3.5 & 0.8 & 0.7 & 0.1 & 0.1 & 0.2 & 0.0 & 0.0  \\
Normalization of $\pi^0$  & 4.0 & 2.6 & 1.7 & 0.2 & 0.1 & 0.1 & 0.0 & 0.0  \\
Particle ID               & 0.1 & 0.1 & 0.0 & 1.1 & 0.7 & 0.5 & 5.3 & 3.9  \\
Momentum resolution       & 1.7 & 0.2 & 0.4 & 0.1 & 0.4 & 0.2 & 0.2 & 0.6  \\
Momentum scale            & 6.1 & 3.4 & 2.0 & 1.0 & 3.1 & 6.2 & 3.9 & 9.5  \\
Angle bias                & 0.6 & 0.5 & 0.2 & 0.3 & 1.3 & 1.0 & 0.9 & 1.6  \\
\bf{Total systematics}    & 9.3 & 6.4 & 4.9 & 3.6 & 4.9 & 7.0 & 6.9 &10.7  \\
\bf{Statistics}           & 1.3 & 1.2 & 1.4 & 1.0 & 1.4 & 2.5 & 1.2 & 2.1  \\
%12
\hline
\bf{12 \GeVc beam}&&&&&&&&\\
\hline
Absorption                & 1.2 & 1.2 & 1.5 & 0.5 & 0.4 & 0.4 & 0.3 & 0.4  \\
Tertiaries                & 1.7 & 3.3 & 3.7 & 1.8 & 2.7 & 2.3 & 0.1 & 0.4  \\
Target region cut         & 3.6 & 1.7 & 1.8 & 2.2 & 1.0 & 0.5 & 1.2 & 0.8  \\
Efficiency                & 1.8 & 2.3 & 1.6 & 1.1 & 2.4 & 2.8 & 1.2 & 2.8  \\
Shape of $\pi^0$          & 4.0 & 0.4 & 1.1 & 0.2 & 0.1 & 0.2 & 0.0 & 0.0  \\
Normalization of $\pi^0$  & 4.1 & 2.5 & 1.8 & 0.3 & 0.1 & 0.1 & 0.1 & 0.0  \\
Particle ID               & 0.1 & 0.1 & 0.0 & 1.1 & 0.6 & 0.2 & 5.1 & 4.1  \\
Momentum resolution       & 1.7 & 0.8 & 0.1 & 0.1 & 0.7 & 0.9 & 0.4 & 0.7  \\
Momentum scale            & 6.4 & 3.7 & 2.4 & 1.2 & 2.3 & 5.5 & 3.5 & 9.2  \\
Angle bias                & 0.5 & 0.5 & 0.3 & 0.4 & 1.1 & 0.9 & 0.9 & 1.8  \\
\bf{Total systematics}    & 9.9 & 6.5 & 5.7 & 3.5 & 4.6 & 6.8 & 6.5 &10.7  \\
\bf{Statistics}           & 1.6 & 1.5 & 1.9 & 1.2 & 1.8 & 3.3 & 1.4 & 2.5  \\
\end{tabular}
\end{center}
}
\end{table}
%


==> Sn5_table1.tex <==
% tin 
\begin{table}[tbp!] 
\caption{Total number of events and tracks used in the tin 
  5\%~$\lambda_{\mathrm{I}}$ target data sets, and the number of
  protons on target as calculated from the pre-scaled trigger count.} 
\label{tab:events}
\begin{center}
\begin{tabular}{ l  r  r r r} \hline
\bf{Data set}&\bf{3 \bfGeVc}&\bf{5 \bfGeVc}&\bf{8 \bfGeVc}&\bf{12 \bfGeVc}\\ \hline
    Total events taken by the DAQ                       & 1636933  & 2827930  & 2780036  &  950582  \\
    Protons on target (selected minimum bias$\times$64) & 1379008  & 4598848  & 8260544  & 3842112  \\
    Accepted protons with interaction triggers          &  263096  &  592960  & 1027142  &  485771  \\
    Accepted protons with Large Angle Int. (LAI)        &   83549  &  304949  &  600581  &  295053  \\
    Maximum \evtspill                                   &     110  &     110  &     120  &     110  \\
    LAI in accepted part of the spill                   &   30029  &   98078  &  199209  &  100872  \\
    Fraction of triggers used                           &    36\%  &    32\%  &    33\%  &    34\%  \\
    LA tracks with $\ge 12$ hits                        &   57076  &  256448  &  662719  &  389780  \\
    Average multiplicity                                &     2.4  &     3.5  &     4.7  &     5.7  \\
    Accepted momentum (vertex constraint)               &   42949  &  188994  &  481436  &  274700  \\
    From target and in kinematic region                 &   29090  &  125864  &  305214  &  167137  \\
    Negative particles                                  &    3352  &   20721  &   63846  &   39395  \\
    Positive particles                                  &   25738  &  105143  &  241368  &  127742  \\
    \bf{$\bfpim$ selected with PID}                     &    3100  &   18762  &   56697  &   34595  \\
    \bf{$\bfpip$ selected with PID}                     &    4439  &   23402  &   64410  &   38009  \\
\end{tabular}
\end{center}
\end{table}
% counters of target.py used:
% #11
% #41 x64
% #21
% #22
% nevt
% #23
% #23/#22
% #72
% mult (mean of trk_mult1 in ..target.aida)
% #84
% #87
% #91
% #92
% #88
% #89



